Implementation of an efficient Bayesian search for gravitational wave bursts with memory in pulsar timing array data

The standard Bayesian technique for searching pulsar timing data for gravitational wave (GW) bursts with memory (BWMs) using Markov Chain Monte Carlo (MCMC) sampling is very computationally expensive to perform. In this paper, we explain the implementation of an efficient Bayesian technique for searching for BWMs. This technique makes use of the fact that the signal model for Earth-term BWMs (BWMs passing over the Earth) is fully factorizable. We estimate that this implementation reduces the computational complexity by a factor of 100. We also demonstrate that this technique gives upper limits consistent with published results using the standard Bayesian technique, and may be used to perform all of the same analyses that standard MCMC techniques can perform.

==> temp.tex <==
The computational complexity of the Bayesian method described in \citetalias{aggarwal_nanograv_2020} depends primarily on the sampling scheme and the complexity involved in inverting the covariance matrix, which contains all parameters that describe the processes in \autoref{eqn:likelihood}. For a single pulsar, the complexity of inverting the matrix in the likelihood calculation goes as $\propto (N_M)^3$ where $N_M$ is the total number of Gaussian Process parameters needed to model the full PTA \citep{ellis_justin_a_enterprise_2020}. The number of total model parameters can be thought of as $N_{psr}  M$, the product of the number of pulsars $N_{psr}$ with the average number of model parameters per pulsar $M$. Normally, inverting a matrix of this size has a computational complexity of $(N_{psr} M)^3$. However, if our signal model contains no correlated signal between pulsar pairs (such as the BWM model described in this paper), the covariance matrix has a block-diagonal structure. We may take advantage of this and reduce the complexity of a single covariance matrix inversion to just $N_{psr}(M)^3$. The number of inversions performed depends on the number of iterations used by the Monte Carlo sampler per run, $N_{iter}$, and the number of runs performed. In general, this is $N_{\Omega} N_{\psi} N_t$, the product of the number of trial burst sky positions, polarizations and epochs, respectively. In total, the complexity scales as: $N_{psr} (M)^3 N_{\text{iter}} N_{\Omega} N_{\psi} N_t$. 

Using the method described in \autoref{sub:accelerated}, computing the lookup tables requires an inversion costing $M^3$ for each entry in the table. Because we begin with four-dimensional grids, the total cost to compute the lookup tables is $M^3 N_{Arn} N_\gamma N_h N_t$, where $N_{Arn}$ and $N_\gamma$ are the number of trial red-noise amplitudes and trial spectral indices parameterizing the red noise in the timing residuals. The complexity of completing all $N_{\text{psr}}$ lookup tables is then $N_{\text{psr}} M^3 N_{Arn} N_\gamma N_h N_t$. Once the likelihood tables are completed, the global two-dimensional likelihood lookup tables are very fast to compute. 

The method described in \autoref{sub:accelerated} is faster as long as the following holds:
$$\frac{N_{Arn} N_\gamma N_h}{N_{\text{iter}} N_\Omega N_\psi} < 1$$
The quantities $N_{Arn}$, $N_\gamma$, $N_h$, and $N_{\text{psr}}$ are in practice quite close, and are approximately on the order of $10^2$. On the other hand, there is a non-trivial overhead involved in Bayesian sampling. Because the parameter volume is quite large, $N_{\text{iter}}$ must be high enough so that the sampler converges on the the global maximum of the posterior distribution. In practice, this number of samples is on the order of $10^4$. This is the largest contributor to the complexity of the fully sampling-based methodology, and avoiding as much sampling as possible saves many operations. Because the lookup tables are computed on a grid, there also exist several methods to expedite this further, such as using vectorization or just-in-time compiling. These were not implemented for computing the results in this paper, and are expected to give an additional significant speedup to this technique.

As pulsar timing arrays grow larger and larger, this will quickly make the fully MCMC-sampled technique unfeasible. For example, \citetalias{aggarwal_nanograv_2020} used 34 pulsars, and the subsequent 12.5-year data release, \citet{alam_nanograv_2020} includes 45 pulsars, giving a factor of approximately 1.75 times higher clock time when using the traditional MCMC technique. On the local high-performance computing cluster available to us, we estimate that the traditional MCMC technique would have taken approximately two years. This more efficient method is able to be completed in approximately three weeks on one consumer-grade desktop machine.
